POPCat: Propagation of particles for complex annotation tasks

Novel dataset creation for all multi-object tracking, crowd-counting, and industrial-based videos is arduous and time-consuming when faced with a unique class that densely populates a video sequence. We propose a time efficient method called POPCat that exploits the multi-target and temporal features of video data to produce a semi-supervised pipeline for segmentation or box-based video annotation. The method retains the accuracy level associated with human level annotation while generating a large volume of semi-supervised annotations for greater generalization. The method capitalizes on temporal features through the use of a particle tracker to expand the domain of human-provided target points. This is done through the use of a particle tracker to reassociate the initial points to a set of images that follow the labeled frame. A YOLO model is then trained with this generated data, and then rapidly infers on the target video. Evaluations are conducted on GMOT-40, AnimalTrack, and Visdrone-2019 benchmarks. These multi-target video tracking/detection sets contain multiple similar-looking targets, camera movements, and other features that would commonly be seen in "wild" situations. We specifically choose these difficult datasets to demonstrate the efficacy of the pipeline and for comparison purposes. The method applied on GMOT-40, AnimalTrack, and Visdrone shows a margin of improvement on recall/mAP50/mAP over the best results by a value of 24.5%/9.6%/4.8%, -/43.1%/27.8%, and 7.5%/9.4%/7.5% where metrics were collected.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> sec/5_limits_future_work.tex <==
\section{Future Work}
\label{sec:future-work}
Future work on the pipeline would include the testing and potential selection of PIPS vs TAPIR based point propagation. TAPIR propagates points faster than PIPs, and utilized appearance augmented tracking. This may allow for re-identification of targets later in the video sequence or identification of new targets that are optically similar. Appearance based filtering of generated examples should be implemented prior to detector training in the future.


==> sec/OLD_STUFF.tex <==
From related work
\subsection{Point Tracking}
%Dheeraj To DO
%Computationally efficient and robust point tracking has been a challenging problem. 
Early methods in pixel-level tracking \cite{inproceedings,teed2020raft} worked with consecutive frames and were efficient to work with slow moving scenes and short-term tracking. They fail to adapt to dynamic scenes and highly occluded environments. Recent methods introduced in the past few years \cite{doersch2022tap,harley2022particle,doersch2023tapir,wang2023tracking} have gained attention due to their ability to maintain long-term tracks in moderate-level occlusions. Persistent Independent Particles (PIPs)\cite{harley2022particle} achieves long term tracking through occlusions by leveraging a temporal window of 8 frames. TAPIR\cite{doersch2023tapir} essentially combines the advantages of PIPs and Tap-Net\cite{doersch2022tap} by modifying Tap-Net's initialization and incorporating it with PIPs' temporal refinement. Although TAPIR achieves higher benchmarks on several datasets, it fails to generalize on sequences with multiple identical small-size objects in a frame and jumps the tracked points from one target to another.

%\subsection{Label Propagation Methods}
%\label{subsec:label-propogation}
%Several methods such as \cite{scalelabel,doersch2023tapir,autotrack,imagenet} take advantage of propagating fewer annotations to multiple frames through different techniques. Autotrack\cite{autotrack} utilizes the GUI of CVAT\cite{CVAT} and integrates it with trackers like ATOM\cite{danelljan2019atom}, KCF\cite{henriques2014high} to annotate short-term tracking datasets. \cite{scalelabel} verifies a few segmentation masks with different scores with the help of human intervention and propagates the likes of good quality masks over the rest of the dataset cluster for the corresponding class.  

\subsection{Segmentation Tracking}
A potential solution to the proposed problem is the area of segmentation tracking, which involves tracking an initialized mask across a sequence. The following algorithms were part of the literature review: Segment Anything Meets Point Tracking(SAM-PT) \cite{rajivc2023segment}, Track Anything Model (TAM) \cite{yang2023track}, and SAM-Track\cite{cheng2023segment}. Optical-flow-based methods\cite{opflow}  failed to handle simultaneous camera and target movements and were therefore not considered. 

SAM-PT\cite{rajivc2023segment} is a mask propagation algorithm that utilizes PIPs\cite{harley2022particle} with Segment Anything Masking\cite{kirillov2023segany} to propagate an instantiated mask across a video sequence. At each frame, the points are retrieved from PIPs and require prompts for the SAM method to mask the target\cite{rajivc2023segment}. The sampling-segmentation-propagation process is chained together to allow for the long-term propagation of masks\cite{rajivc2023segment}. SAM-PT requires multiple positive point selections along with negative points to initialize a mask. This process is too laborious for multi-target scenarios which was why SAM-PT could not be considered for our pipeline.

Track Anything Model (TAM)\cite{yang2023track}  is a video object segmentation (VOS) work that leverages SAM for masking and XMem\cite{cheng2022xmem} for video segmentation. The authors exploited the high accuracy of SAM masks to boost the precision of XMem\cite{cheng2022xmem} VOS\cite{yang2023track}. TAM does not require training on the tested dataset and is instantiated by a prompted initial SAM mask. TAM was incompatible with our proposed solution as it does not support new object segmentation.

%Space-time correspondence as a Contrastive Random Walk\cite{NEURIPS2020_e2ef524f} was a VOS paper which propagated a query mask across a set of frames. This work was noted for its unique use of palindromes sequences in frame motion as a means of self-supervision in training\cite{NEURIPS2020_e2ef524f}. The model utilizes an embedding matrix with soft attention to build a space-time graph that defines the image as nodes\cite{NEURIPS2020_e2ef524f}. CRW was impractical for our use case as it required significant computing power and was too slow for long-duration videos.

SAM-Track\cite{cheng2023segment} is a VOS tracker that utilizes a semantic detector to integrate new detections using Grounding-Dino\cite{liu2023grounding} with a first frame annotation. DeAOT\cite{yang2022decoupling} was used for multi-target tracking within the algorithm, and interactive user input is available\cite{cheng2023segment}. SAM-Track could not be used within the pipeline as it relied on semantic modules for new object detection.

Overall, segmentation-based tracking was reviewed and eliminated as a potential solution to generic object annotation. It was understood that tracking through segmentation would not be computationally efficient nor effective for the goal set for our system.


\subsection{Box Resizing}
A literature review of box resizing methods identified GrabCut \cite{grabcut} and Autofit\cite{autofit} as iterative resizing methods.
Grabcut\cite{grabcut} requires an input bounding rectangle which completely encompasses the target region. The algorithm then iteratively segments the image and allows the user to mask the image through the use of exclusionary strokes \cite{grabcut}. Grabcut was not applicable for the pipeline as it requires manual inputs to achieve acceptable results.
Autofit \cite{autofit} utilizes a background subtraction with Grabcut between consecutive frames to identify the moving target areas of the image. The algorithm generates a foreground mask, calculates the extent of the box based on the foreground mask, and then generates a new box based on said calculations\cite{autofit}. Autofit required high compute resources in the multi-target annotation case and was deemed ill-suited to our requirements.
We instead augmented our use of SAM by applying a minimal bounding box to the masks generated for segmentation training. This resulted in boxes resized to the generated mask at a negligible computational cost. The process is explained in section \ref{subsubsec:BBS}, and is depicted in (C) of Fig. \ref{fig:pipeline}.




Segment Anything Model (SAM)\cite{kirillov2023segany} is a zero-shot segmentation model that has the capability of creating segmentation masks based on the selected points, selected rectangles, or even mentioned text prompts in a given frame. Once the centers of the annotated bounding boxes are propagated through PIPs, SAM\cite{kirillov2023segany} uses the roughly annotated bounding boxes and accurately creates the segmentation masks for all the frames. These segmentation masks are then used to further extract precise bounding boxes across the frames for all the objects by obtaining the minimum fitted bounding box rectangle on the segmentation contour. In addition to segmentation masks, this module supplies box outputs for downstream training. Given that SAM is a foundational model, it requires no further training to effect accurate segmentation masks. A careful review of the failure cases of SAM in \cite{ji2023segment} shows no failure modes that adversely affect the intended use case. A box is applied around the target to eliminate much of the over-or-under segmentation issues associated with SAM \cite{ji2023segment}. 

% Furthermore, a prompt is provided with each box to allow for accurate association of segmentation masks to the intended target. 
The application of SAM is shown in (C) of Fig. \ref{fig: pipeline} and represented in Algorithm \ref{alg:pipeline_alg} lines 9-12. This includes the extraction of segmentation masks and the creation of fitted bounding boxes.

The reasoning behind box resizing is grounded in literature, with algorithms such as Grabcut \cite{grabcut} or Autofit \cite{autofit} showing increased precision and recall as a direct result of enhanced bounding boxes. Further discussion of box resizing requires empirical analysis and is under the ablation study in section \ref{subsubsec:SAMAPPS}. The bounding boxes and masks generated in the segmentation portion of the pipeline are saved and passed on to the final stage for training.

The stages prescribed above are represented in Algorithm \ref{alg:pipeline_alg}. The algorithm can be repeated for any number of annotation-sequence pairs as provided. The provision of more pairs would result in better coverage and more accurate annotation of the target video.
